Photochemistry and Spectral Characterization of Temperate and Gas-Rich Exoplanets

Exoplanets that receive stellar irradiance of approximately Earth's or less have been discovered and many are suitable for spectral characterization. Here we focus on the temperate planets that have massive H2-dominated atmospheres, and trace the chemical reactions and transport following the photodissociation of H2O, CH4, NH3, and H2S, with K2-18 b, PH2 b, and Kepler-167 e representing temperate/cold planets around M and G/K stars. We find that NH3 is likely depleted by photodissociation to the cloud deck on planets around G/K stars but remains intact in the middle atmosphere of planets around M stars. A common phenomenon on temperate planets is that the photodissociation of NH3 in presence of CH4 results in HCN as the main photochemical product. The photodissociation of CH4 together with H2O leads to CO and CO2, and the synthesis of hydrocarbon is suppressed. Temperate planets with super-solar atmospheric metallicity and appreciable internal heat may have additional CO and CO2 from the interior and less NH3 and thus less HCN. Our models of K2-18 b can explain the transmission spectrum measured by Hubble, and indicate that future observations in 0.5-5.0 um would provide the sensitivity to detect the equilibrium gases CH4, H2O, and NH3, the photochemical gas HCN, as well as CO2 in some cases. Temperate and H2-rich exoplanets are thus laboratories of atmospheric chemistry that operate in regimes not found in the Solar System, and spectral characterization of these planets in transit or reflected starlight promises to greatly expand the types of molecules detected in exoplanet atmospheres.

==> tables.tex <==
	\setcounter{table}{0}
	\begin{deluxetable}{c|cc}
		\tablecaption{Relevant parameters of the studied targets \label{tab:param}}
		\tablehead{
			\colhead{Parameter} 		& 			\colhead{HD189733} 								& 				\colhead{HD209458}												}
		\startdata
		Stellar Parameters 				&  															&  																			\\
		\hline
		$R_{\star}$ (R$_{\odot}$)			&			$0.756 \pm 0.018$			\tablenotemark{1}			&				($1.155_{-0.016}^{+0.014}$)			\tablenotemark{1}				\\
		$T_{eff}$ (K) 					&			$5040 \pm 50$				\tablenotemark{1}			&				$6065 \pm 50$						\tablenotemark{1} 				\\
		$M_{\star}$ (M$_{\odot}$)			&			$0.806 \pm 0.048$			\tablenotemark{1}			&				$1.119 \pm 0.033$					\tablenotemark{1}				\\
		$log(g_{\star})$ (csg)				&			$4.587 \pm 0.015$			\tablenotemark{1}			&				$4.361 \pm 0.008$					\tablenotemark{1}				\\
		$v_{sys}$ (kms$^{-1}$)			&			$-2.361 \pm 0.003$			\tablenotemark{2}			& 				$-14.7652 \pm 0.0016$				\tablenotemark{5} 				\\
		\hline
		Planet Parameters 				& 															&																			\\
		\hline
		$T_{eq}$ (K)					&			$(1201_{-12}^{+13})$ 		\tablenotemark{1}			&				$1449 \pm 12$						\tablenotemark{1}				\\
		$a$ (AU) 						&			$0.03120(27)$				\tablenotemark{3} 			& 				$(0.04707_{-0.00047}^{+0.00046})$		\tablenotemark{1} 				\\
		$R_p$ (R$_{Jup}$) 				&			$(1.178_{-0.023}^{+0.016})$	\tablenotemark{3}			&				$(1.359_{-0.019}^{+0.016})$			\tablenotemark{1}				\\
		$M_p$ (M$_{Jup}$)				&			$(1.144_{-0.056}^{+0.057})$	\tablenotemark{1}			&				$0.685 \pm 0.015$					\tablenotemark{1}				\\
		$P$ (days)					&			$2.21857567(15)$			\tablenotemark{4} 			& 				$3.52474859(38)$					\tablenotemark{6}				\\
		$T_0$ (BJD$_{UTC}$)			&			$2454279.436714(15)$		\tablenotemark{4}			&				$2452826.629283(87)$				\tablenotemark{6}				\\
		$I$ (deg)						&			$85.710 \pm 0.024$			\tablenotemark{4}			&				$86.71 \pm 0.05$					\tablenotemark{1}				\\ 
		\enddata
		\tablecomments{$^1$\cite{Torres2008}, $^2$\cite{Bouchy2005}, $^3$\cite{Triaud2009}, $^4$\cite{Agol2010}, $^5$\cite{Mazeh2000}, $^6$\cite{Knutson2007}}
	\end{deluxetable}
		
		
	\begin{deluxetable}{c|cc}
		\tablecaption{This work and previous results \label{tab:results}}
		\tablehead{
			\colhead{Parameter} 		& 			\colhead{HD189733} 								& 				\colhead{HD209458}												}
		\startdata
		\hline
		Previous results			 	& 			\cite{Brogi2016}									& 				\cite{Snellen2010}												\\
		\hline
		SNR$_{CO}$					&			-												&				-															\\
		$K_{p,\ CO}$ (kms$^{-1}$)		&			$205_{-51}^{+38}$									&				-															\\
		$v_{p,\ CO}$ (kms$^{-1}$)			&			-												&				$140 \pm 10$													\\
		$v_{rest,\ CO}\ $(kms$^{-1}$)		&			$-1.6_{-1.8}^{+2.0}$									&				$\sim$ 2														\\
		SNR$_{H{_2}O}$				&			5.5												&				-															\\
		$K_{p,\ H{_2}O}$ (kms$^{-1}$)		&			$183_{-59}^{+38}$									&				-															\\
		$v_{rest,\ H{_2}O}\ $(kms$^{-1}$)	&			$-1.58_{-1.50}^{+1.65}$								&				-															\\
		\hline
		Results						& 			This Work											&				This Work														\\
		\hline
		SNR$_{CO}$					&			5.24												&				5.7															\\
		$K_{p,\ CO}$ (kms$^{-1}$)		&			$190	 \pm 16$										&				$148_{-15}^{+16}$												\\
		$v_{rest,\ CO}\ $(kms$^{-1}$)		&			$-3.0_{-1.3}^{+1.0}$									&				$-3.0_{-1.1}^{+1.3}$												\\
		W T-Test$_{CO}$ ($\sigma$)		&			-												&				21.62														\\
		SNR$_{H{_2}O}$				&			3.69												&				3.95															\\
		$K_{p,\ H{_2}O}$ (kms$^{-1}$)		&			$167_{-21}^{+32}$									&				$140_{-16}^{+25}$												\\
		$v_{rest,\ H{_2}O}\ $(kms$^{-1}$)	&			$-4.0_{-1.8}^{+2.0}$									&				$-4.0_{-1.6}^{+1.4}$												\\
		W T-Test$_{H{_2}O}$ ($\sigma$)	&			5.21												&				6.56															\\
		\enddata
	\end{deluxetable}

==> widetab.tex <==
\begin{longrotatetable}
\begin{deluxetable}{lllrrrrrrll}
\tablecaption{Observable Characteristics of 
Galactic/Magellanic Cloud novae with X-ray observations\label{chartable}}
\tablewidth{700pt}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{Name} & \colhead{V$_{max}$} & 
\colhead{Date} & \colhead{t$_2$} & 
\colhead{FWHM} & \colhead{E(B-V)} & 
\colhead{N$_H$} & \colhead{Period} & 
\colhead{D} & \colhead{Dust?} & \colhead{RN?} \\ 
\colhead{} & \colhead{(mag)} & \colhead{(JD)} & \colhead{(d)} & 
\colhead{(km s$^{-1}$)} & \colhead{(mag)} & \colhead{(cm$^{-2}$)} &
\colhead{(d)} & \colhead{(kpc)} & \colhead{} & \colhead{}
} 
\startdata
CI Aql & 8.83 (1) & 2451665.5 (1) & 32 (2) & 2300 (3) & 0.8$\pm0.2$ (4) & 1.2e+22 & 0.62 (4) & 6.25$\pm5$ (4) & N & Y \\
{\bf CSS081007} & \nodata & 2454596.5 & \nodata & \nodata & 0.146 & 1.1e+21 & 1.77 (5) & 4.45$\pm1.95$ (6) & \nodata & \nodata \\
GQ Mus & 7.2 (7) & 2445352.5 (7) & 18 (7) & 1000 (8) & 0.45 (9) & 3.8e+21  & 0.059375 (10) & 4.8$\pm1$ (9) & N (7) & \nodata \\
IM Nor & 7.84 (11) & 2452289 (2) & 50 (2) & 1150 (12) & 0.8$\pm0.2$ (4) & 8e+21 & 0.102 (13) & 4.25$\pm3.4$ (4) & N & Y \\
{\bf KT Eri} & 5.42 (14) & 2455150.17 (14) & 6.6 (14) & 3000 (15) & 0.08 (15) & 5.5e+20 & \nodata & 6.5 (15) & N & M \\
{\bf LMC 1995} & 10.7 (16) & 2449778.5 (16) & 15$\pm2$ (17) & \nodata & 0.15 (203) & 7.8e+20  & \nodata & 50 & \nodata & \nodata \\
LMC 2000 & 11.45 (18) & 2451737.5 (18) & 9$\pm2$ (19) & 1700 (20) & 0.15 (203) & 7.8e+20  & \nodata & 50 & \nodata & \nodata \\
{\bf LMC 2005} & 11.5 (21) & 2453700.5 (21) & 63 (22) & 900 (23) & 0.15 (203) & 1e+21 & \nodata & 50  & M (24) & \nodata \\
{\bf LMC 2009a} & 10.6 (25) & 2454867.5 (25) & 4$\pm1$  & 3900 (25) & 0.15 (203)  & 5.7e+20 & 1.19 (26) & 50 & N & Y \\
{\bf SMC 2005} & 10.4 (27) & 2453588.5 (27) & \nodata & 3200 (28) & \nodata & 5e+20  & \nodata & 61 & \nodata & \nodata \\
{\bf QY Mus} & 8.1 (29) & 2454739.90 (29) & 60:  & \nodata & 0.71 (30) & 4.2e+21  & \nodata & \nodata & M & \nodata \\
{\bf RS Oph} & 4.5 (31) & 2453779.44 (14) & 7.9 (14) & 3930 (31) & 0.73 (32) & 2.25e+21 & 456 (33) & 1.6$\pm0.3$ (33) & N (34) & Y \\
{\bf U Sco} & 8.05 (35) & 2455224.94 (35) & 1.2 (36) & 7600 (37) & 0.2$\pm0.1$ (4) & 1.2e+21 & 1.23056 (36) & 12$\pm2$ (4) & N & Y \\
{\bf V1047 Cen} & 8.5 (38) & 2453614.5 (39) & 6 (40) & 840 (38) & \nodata & 1.4e+22  & \nodata & \nodata & \nodata & \nodata \\
{\bf V1065 Cen} & 8.2 (41) & 2454123.5 (41) & 11 (42) & 2700 (43) & 0.5$\pm0.1$ (42) & 3.75e+21 & \nodata & 9.05$\pm2.8$ (42) & Y (42) & \nodata \\
V1187 Sco & 7.4 (44) & 2453220.5 (44) & 7: (45) & 3000 (44) & 1.56 (44) & 8.0e+21 & \nodata & 4.9$\pm0.5$ (44) & N & \nodata \\
{\bf V1188 Sco} & 8.7 (46) & 2453577.5 (46) & 7 (40) & 1730 (47) & \nodata & 5.0e+21  & \nodata & 7.5 (39) & \nodata & \nodata \\
{\bf V1213 Cen} & 8.53 (48) & 2454959.5 (48) & 11$\pm2$ (49) & 2300 (50) & 2.07 (30) & 1.0e+22 & \nodata & \nodata & \nodata & \nodata \\
{\bf V1280 Sco} & 3.79 (51) & 2454147.65 (14) & 21 (52) & 640 (53) & 0.36 (54) & 1.6e+21  & \nodata & 1.6$\pm0.4$ (54) & Y (54) & \nodata \\
{\bf V1281 Sco} & 8.8 (55) & 2454152.21 (55) & 15:& 1800 (56) & 0.7 (57) & 3.2e+21 & \nodata & \nodata & N & \nodata \\
{\bf V1309 Sco} & 7.1 (58) & 2454714.5 (58) & 23$\pm2$ (59) & 670 (60) & 1.2 (30) & 4.0e+21 & \nodata & \nodata & \nodata & \nodata \\
{\bf V1494 Aql} & 3.8 (61) & 2451515.5 (61) & 6.6$\pm0.5$ (61) & 1200 (62) & 0.6 (63) & 3.6e+21  & 0.13467 (64) & 1.6$\pm0.1$ (63) & N & \nodata \\
{\bf V1663 Aql} & 10.5 (65) & 2453531.5 (65) & 17 (66) & 1900 (67) & 2: (68) & 1.6e+22  & \nodata & 8.9$\pm3.6$ (69) & N & \nodata \\
V1974 Cyg & 4.3 (70) & 2448654.5 (70) & 17 (71) & 2000 (19) & 0.36$\pm0.04$ (71) & 2.7e+21  & 0.081263 (70) & 1.8$\pm0.1$ (72) & N & \nodata \\
{\bf V2361 Cyg} & 9.3 (73) & 2453412.5 (73) & 6 (40) & 3200 (74) & 1.2: (75) & 7.0e+21 & \nodata & \nodata & Y (40) & \nodata \\
{\bf V2362 Cyg} & 7.8 (76) & 2453831.5 (76) & 9 (77) & 1850 (78) & 0.575$\pm0.015$ (79) & 4.4e+21  & 0.06577 (80) & 7.75$\pm3$ (77) & Y (81) & \nodata \\
{\bf V2467 Cyg} & 6.7 (82) & 2454176.27 (82) & 7 (83) & 950 (82) & 1.5 (84) & 1.4e+22  & 0.159 (85) & 3.1$\pm0.5$ (86) & M (87) & \nodata \\
{\bf V2468 Cyg} & 7.4 (88) & 2454534.2 (88) & 10: & 1000 (88) & 0.77 (89) & 1.0e+22  & 0.242 (90) & \nodata & N & \nodata \\
{\bf V2491 Cyg} & 7.54 (91) & 2454567.86 (91) & 4.6 (92) & 4860 (93) & 0.43 (94) & 4.7e+21  & 0.09580: (95) & 10.5 (96) & N & M \\
V2487 Oph & 9.5 (97) & 2450979.5 (97) & 6.3 (98) & 10000 (98) & 0.38$\pm0.08$ (98) & 2.0e+21 & \nodata & 27.5$\pm3$ (99) & N (100) & Y (101) \\
{\bf V2540 Oph} & 8.5 (102) & 2452295.5 (102) & \nodata & \nodata & \nodata & 2.3e+21 & 0.284781 (103) & 5.2$\pm0.8$ (103) & N & \nodata \\
V2575 Oph & 11.1 (104) & 2453778.8 (104) & 20: & 560 (104) & 1.4 (105) & 3.3e+21 & \nodata & \nodata & N (105) & \nodata \\
{\bf V2576 Oph} & 9.2 (106) & 2453832.5 (106) & 8: & 1470 (106) & 0.25 (107) & 2.6e+21  & \nodata & \nodata & N & \nodata \\
{\bf V2615 Oph} & 8.52 (108) & 2454187.5 (108) & 26.5 (108) & 800 (109) & 0.9 (108) & 3.1e+21  & \nodata & 3.7$\pm0.2$ (108) & Y (110) & \nodata \\
{\bf V2670 Oph} & 9.9 (111) & 2454613.11 (111) & 15: & 600 (112) & 1.3: (113) & 2.9e+21  & \nodata & \nodata & N (114) & \nodata \\
{\bf V2671 Oph} & 11.1 (115) & 2454617.5 (115) & 8: & 1210 (116) & 2.0 (117) & 3.3e+21  & \nodata & \nodata & M (117) & \nodata \\
{\bf V2672 Oph} & 10.0 (118) & 2455060.02 (118) & 2.3 (119) & 8000 (118) & 1.6$\pm0.1$ (119) & 4.0e+21  & \nodata & 19$\pm2$ (119) & \nodata & M \\
V351 Pup & 6.5 (120) & 2448617.5 (120) & 16 (121) & \nodata & 0.72$\pm0.1$ (122) & 6.2e+21 & 0.1182 (123) & 2.7$\pm0.7$ (122) & N & \nodata \\
{\bf V382 Nor} & 8.9 (124) & 2453447.5 (124) & 12 (40) & 1850 (23) & \nodata & 1.7e+22 & \nodata & \nodata & \nodata & \nodata \\
V382 Vel & 2.85 (125) & 2451320.5 (125) & 4.5 (126) & 2400 (126) & 0.05: (126) & 3.4e+21  & 0.146126 (127) & 1.68$\pm0.3$ (126) & N & \nodata \\
{\bf V407 Cyg} & 6.8 (128) & 2455266.314 (128) & 5.9 (129) & 2760 (129) & 0.5$\pm0.05$ (130) & 8.8e+21 & 15595 (131) & 2.7 (131) & \nodata & Y \\
{\bf V458 Vul} & 8.24 (132) & 2454322.39 (132) & 7 (133) & 1750 (134) & 0.6 (135) & 3.6e+21 & 0.06812255 (136) & 8.5$\pm1.8$ (133) & N (135) & \nodata \\
{\bf V459 Vul} & 7.57 (137) & 2454461.5 (137) & 18 (138) & 910 (139) & 1.0 (140) & 5.5e+21  & \nodata & 3.65$\pm1.35$ (138) & Y (140) & \nodata \\
V4633 Sgr & 7.8 (141) & 2450895.5 (141) & 19$\pm3$ (142) & 1700 (143) & 0.21 (142) & 1.4e+21  & 0.125576 (144) & 8.9$\pm2.5$ (142) & N & \nodata \\
{\bf V4643 Sgr} & 8.07 (145) & 2451965.867 (145) & 4.8 (146) & 4700 (147) & 1.67 (148) & 1.4e+22 & \nodata & 3 (148) & N & \nodata \\
{\bf V4743 Sgr} & 5.0 (149) & 2452537.5 (149) & 9 (150) & 2400 (149) & 0.25 (151) & 1.2e+21 & 0.281 (152) & 3.9$\pm0.3$ (151) & N & \nodata \\
{\bf V4745 Sgr} & 7.41 (153) & 2452747.5 (153) & 8.6 (154) & 1600 (155) & 0.1 (154) & 9.0e+20  & 0.20782 (156) & 14$\pm5$ (154) & \nodata & \nodata \\
{\bf V476 Sct} & 10.3 (157) & 2453643.5 (157) & 15 (158) & \nodata & 1.9 (158) & 1.2e+22  & \nodata & 4$\pm1$ (158) & M (159) & \nodata \\
{\bf V477 Sct} & 9.8 (160) & 2453655.5 (160) & 3 (160) & 2900 (161) & 1.2: (162) & 4e+21  & \nodata & \nodata & M (163) & \nodata \\
{\bf V5114 Sgr} & 8.38 (164) & 2453081.5 (164) & 11 (165) & 2000 (23) & \nodata & 1.5e+21  & \nodata & 7.7$\pm0.7$ (165) & N (166) & \nodata \\
{\bf V5115 Sgr} & 7.7 (167) & 2453459.5 (167) & 7 (40) & 1300 (168) & 0.53 (169) & 2.3e+21  & \nodata & \nodata & N (169) & \nodata \\
{\bf V5116 Sgr} & 8.15 (170) & 2453556.91 (170) & 6.5 (171) & 970 (172) & 0.25 (173) & 1.5e+21 & 0.1238 (171) & 11$\pm3$ (173) & N (174) & \nodata \\
{\bf V5558 Sgr} & 6.53 (175) & 2454291.5 (175) & 125 (176) & 1000 (177) & 0.80 (178) & 1.6e+22  & \nodata & 1.3$\pm0.3$ (176) & N (179) & \nodata \\
{\bf V5579 Sgr} & 5.56 (180) & 2454579.62 (180) & 7: & 1500 (23) & 1.2 (181) & 3.3e+21 & \nodata & \nodata & Y (181) & \nodata \\
{\bf V5583 Sgr} & 7.43 (182) & 2455051.07 (182) & 5: & 2300 (182) & 0.39 (30) & 2.0e+21 & \nodata & 10.5 & \nodata & \nodata \\
{\bf V574 Pup} & 6.93 (183) & 2453332.22 (183) & 13 (184) & 2800 (184) & 0.5$\pm0.1$  & 6.2e+21 & \nodata & 6.5$\pm1$  & M (185) & \nodata \\
{\bf V597 Pup} & 7.0 (186) & 2454418.75 (186) & 3: & 1800 (187) & 0.3 (188) & 5.0e+21  & 0.11119 (189) & \nodata & N (188) & \nodata \\
{\bf V598 Pup} & 3.46 (14) & 2454257.79 (14) & 9$\pm1$ (190) & \nodata & 0.16 (190) & 1.4e+21 & \nodata & 2.95$\pm0.8$ (190) & \nodata & \nodata \\
{\bf V679 Car} & 7.55 (191) & 2454797.77 (191) & 20: & \nodata & \nodata & 1.3e+22  & \nodata & \nodata & \nodata & \nodata \\
{\bf V723 Cas} & 7.1 (192) & 2450069.0 (192) & 263 (2) & 600 (193) & 0.5 (194) & 2.35e+21  & 0.69 (195) & 3.86$\pm0.23$ (196) & N & \nodata \\
V838 Her & 5 (197) & 2448340.5 (197) & 2 (198) & \nodata & 0.5$\pm0.1$ (198) & 2.6e+21  & 0.2975 (199) & 3$\pm1$ (198) & Y (200) & \nodata \\
{\bf XMMSL1 J06} & 12 (201) & 2453643.5 (202) & 8$\pm2$ (202) & \nodata & 0.15 (203) & 8.7e+20 & \nodata & 50 & \nodata & \nodata \\
\enddata
\end{deluxetable}
\end{longrotatetable}

